Learning and Planning for Temporally Extended Tasks in Unknown Environments

We propose a novel planning technique for satisfying tasks specified in temporal logic in partially revealed environments. We define high-level actions derived from the environment and the given task itself, and estimate how each action contributes to progress towards completing the task. As the map is revealed, we estimate the cost and probability of success of each action from images and an encoding of that action using a trained neural network. These estimates guide search for the minimum-expected-cost plan within our model. Our learned model is structured to generalize across environments and task specifications without requiring retraining. We demonstrate an improvement in total cost in both simulated and real-world experiments compared to a heuristic-driven baseline.

==> defining_the_action_set.tex <==
% Chris attempt (built off Greg's)
The set of actions available to the robot at any moment depends on its state in the product automaton given by the current map and the \gls{dfa} defined by the task specification. As discussed in section \ref{sub:dfa-preliminaries}, a \gls{dfa} represents the robot's specified task at a high level, and allows the robot to keep track of its progress through a task that would otherwise be non-markov. The product automaton $\mathcal{A}^P$ constructed from a given \gls{dfa} and the robot's map fully defines the ways a robot can plan to transition through the \gls{dfa} accomplish its task. As the robot explores its environment, it may discover that it can satisfy its task completely in known space by planning through $\mathcal{A}^P$. For example, if the robot already knows where the fire and exit are located in the map, once it finds the extinguisher, it would be able to plan a trajectory in the product automaton which reaches an accepting state, thus satisfying its specification completely in known space.

However, in our problem setting, the map is only partially revealed at the outset, and the agent must consider that there may be extinguishers and alarms and fires that have not yet been discovered. Planning to solve any task in partially explored environments can be modelled as a POMDP, as mentioned above, and so the expected cost of taking the optimal action can be computed using the Bellman Equation. An important insight in \cite{Stein2018} is that, though this computation is intractable in general, if we define useful high-level actions and divide future belief state after an action into cases where it either succeeds or fails, we can greatly reduce the complexity of the computation.

We thus define our action set similar to \citep{Stein2018}, with the caveat that our subgoals plan to complete a single transition in the \gls{dfa} in unknown space, instead of an entire task. Specifically, the robot can plan through its product automaton to a point along a \emph{frontier}---the contiguous boundaries between free and unknown space---then enter unknown space beyond that frontier to attempt to transition to a new state in the \gls{dfa}. If turning on the alarm is relevant to the robot's task, for example, it could choose any of the frontiers, and travel through that frontier with the intent of finding and activating an alarm (while avoiding the fire). Since we use $\mathcal{A}^P$ to plan to a frontier in known space, the robot can progress through the \gls{dfa} as it travels to the chosen frontier. Continuing our example, if the robot has revealed a fire extinguisher, one subgoal would be to try to find the fire beyond a particular frontier, picking up the extinguisher along the way. Thus, subgoals can be completely described by the tuple: $a_{f, z, z'} = (f, z, z')$, where $f$ is the frontier of interest, $z$ is the state in the \gls{dfa} after traveling through the product automaton to the frontier, and $z'$ is the state the agent would attempt to reach beyond the frontier. As in \cite{Stein2018}, we also check if the specification can be satisfied in known space, and add that action to our set of subgoals.

At planning time, our agent imagines what the impact will be of executing a high-level action. Though any transitions made in known space are deterministic, subgoals may succeed or fail with some probability. During a planning rollout, the agent imagines that some information about the environment is revealed as it executes exploratory actions. If the agent fails to transition to state $z'$ after imagining execution of $a_{f, z, z'}$, this action is removed from its action set for the remainder of the rollout, since the frontier $f$ is then known not to allow this transition. By contrast, if the action succeeds, the action is guaranteed to succeed again, equivalent to setting the success probability of action $a_{f, z, z'}$ to 1; updating the action's success probability records that the agent has successfully transitioned from $z$ to $z'$ via frontier $f$ and that it could do so again if it were necessary.

% GJStein attempt: 
%- Example: want to find alarm while avoid fire
%- This is a \emph{transition in the DFA}; these transitions correspond to actions the robot can take.
%- When the env is partially revealed, each boundary/frontier provide additional avenues for achieving transitions in the DFA (as a function of what is likely to lie beyond that boundary).
%- Already have sentence: "Specifically, the robot can plan..."

The actions available to our agent are defined by the robot's state in the \gls{dfa}. For example, if to put out the fire our agent needs to activate the sprinklers, each sprinkler control panel we have observed corresponds to a high-level action. However, in our problem setting, the map is only partially revealed, and the agent should also take exploratory actions in search of sprinkler controls that have not yet been discovered. We define our action set similar to \citep{Stein2018}: each \emph{frontier}, a contiguous boundary between free and unknown space, corresponds to one way our agent can leave known space in an effort to transition to a new state in the \gls{dfa}. \todo{[chris] I dont believe this (known and exploratory) accurately represents the subgoals we are considering. Maybe this is where the difference between "high-level actions" and subgoals exists.  For us, a subgoal is not, flip the alarm because I can see it (unless that completes the specification). Instead, the subgoal is "flip the alarm, then try to find the exit through this frontier."} Therefore, in addition to the \emph{known actions} defined by the already-revealed portion of the environment, each frontier defines new \emph{exploratory actions}, one for each possible transition in the \gls{dfa}. [gjstein: I've just pasted this; it probably needs to be molded.] Thus, subgoals can be completely described by the tuple: $a_{f, z, z'} = (f, z, z')$, where $f$ is the frontier of interest, $z$ is the state in the \gls{dfa} after traveling through the product automaton to the frontier, and $z'$ is the state the agent would attempt to reach beyond the frontier (Note: since $(z,z')$ defines a transition $t$, we can equivalently write $a_{f, t}$).

At planning time, our agent imagines what the impact will be of executing a high-level action. Though the known actions are deterministic, the exploratory actions may succeed or fail with some probability. During a planning rollout, the agent imagines that some information about the environment is revealed as it executes exploratory actions. If the agent fails to transition to state $z'$ after imagining execution of $a_{f, z, z'}$, this exploratory action is removed from its action set for the remainder of the rollout, since the frontier $f$ is then known not to allow this transition. By contrast, if the action succeeds, the action is guaranteed to succeed again, equivalent to setting the success probability of action $a_{f, z, z'}$ to 1; updating the action's success probability records that the agent has successfully transitioned from $z$ to $z'$ via frontier $f$ and that it could do so again if it were necessary\todo{[gjstein] Question: this language may need to be cleaned up. Not sure if it covers all our bases.}.

\todo{[chris] I took another crack above this attempt, taking pieces from both}


%% END: gjstein attempt

The set of subgoals available to the robot depends on the product automaton given by the current map, and the robot's state in the \gls{dfa}. Specifically, the robot can plan through its product automaton to a point along a frontier, then enter unknown space beyond that frontier to attempt to transition to a new state in the \gls{dfa}. For example, if the robot is considering turning on the alarm, it could choose any of the frontiers that define the contiguous boundaries between free and unknown space, and travel through that frontier with the intent of finding the alarm, while avoiding the fire to transition in the \gls{dfa}. The probability of this subgoal successfully causing the robot to transition \gls{dfa} states \todo{Question: is the first half of this sentence clear? I worry that we're not being as accessible to non-LTL people as we could be.} depends on the unknown portion of the map, and is estimated by the neural network. Similarly, the costs of success and failure are also estimated by the network. %Note that the action of attempting to find the sprinklers beyond the same frontier is a different subgoal entirely, with different associated costs and probability of success.

%Alternatively, the robot can completely satisfy the \gls{dfa} by reaching an accepting state in known space. For example, if the robot already knows where the fire and exit are located in the map, once it finds the extinguisher, it would be able to plan a trajectory in the product automaton which reaches an accepting state, thus satisfying its specification completely in known space. If such a path exists, this action would have a probability of success of one, and the exact cost of success would be known by planning through the product automaton. 


Using the product automaton, we consider transitions as the robot travels through known space as well. For example, if the robot sees the fire extinguisher, one subgoal would be to try to find the fire beyond a particular frontier, picking up the extinguisher along the way. Thus, subgoals can be completely described by the tuple: $a_{f, z, z'} = (f, z, z')$, where $f$ is the frontier of interest, $z$ is the state in the \gls{dfa} after traveling through the product automaton to the frontier, and $z'$ is the state the agent would attempt to reach beyond the frontier (Note: since $(z,z')$ defines a transition $t$, we can equivalently write $a_{f, t}$). As the robot explores its environment, it may encounter instances where it can satisfy its task completely in known space. For example, if the robot already knows where the fire and exit are located in the map, once it finds the extinguisher, it would be able to plan a trajectory in the product automaton which reaches an accepting state, thus satisfying its specification completely in known space. If such a path exists, this action would have a probability of success of one, and the exact cost of success would be known by planning through the product automaton. 

==> preliminaries_backup.tex <==
\section{Preliminaries}

%\subsection{Syntactically Co-Safe Linear Temporal Logic} \label{sub:ltl-preliminaries}
\glsresetall

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/preliminaries.png}
    \caption{\textbf{Task specification and environment abstraction.} A. The \acrfull{scltl} specification $(\lnot \texttt{fire}\ \mathcal{U}\ (\texttt{alarm})) \vee (\lnot (\texttt{fire}\ \mathcal{U}\ \texttt{extinguisher}) \wedge \lozenge (\texttt{fire})))$ is transformed into a \acrfull{dfa}. B. The environment is abstracted as a \acrfull{wfdts}. C. The product automaton combines the \acrshort{dfa} and \acrshort{wfdts} allowing the robot to construct a plan to solve a specification. \adam{NOTE: This will be changed to match the style of Fig. \ref{fig:defining-actions} with similar, although likely different, information contained.}}
    \label{fig:dfa_ts_pa}
\end{figure}
\end{comment}

% The tasks we consider in this work are not infinite, i.e. they have a definitive ending point.
% We are primarily interested in tasks which can be completed in finite time. As such, we use \gls{scltl} \cite{Kupferman2001} (a variant of LTL) to encode the tasks the robot should accomplish.

We use \gls{scltl} \cite{Kupferman2001}, a fragment of \gls{ltl}, to encode the tasks the robot should accomplish.
\gls{scltl} allows us to specify tasks that can be accomplished in finite time.


% Tasks specificied in \gls{scltl} are able to be completed in finite time, opposed to some variants of \gls{ltl} where tasks are objectives the robot should repeatedly accomplish.
% We use \gls{scltl} to encode the task our robot should accomplish. 
% Using \gls{scltl} we can specify a task for the robot and find what it needs to do to accomplish the task.
% As opposed to some variants of \gls{ltl} where tasks are things the robot should repeatedly do, tasks specified in \gls{scltl} can be completed.
% This type of logic is well suited to the type of scenarios where a robot needs to accomplish a task in a partially unknown environment.
%\chris{maybe a discussion of why}

\paragraph{Syntax and Semantics}
In \gls{scltl}, formulas are written over a set of atomic propositions $\Sigma$ with Boolean and temporal operators \cite{Kupferman2001}.
The Boolean operators are negation ($\lnot$), conjunction ($\wedge$), and disjunction ($\vee$) and the temporal operators are next ($\bigcirc$), until ($\mathcal{U}$), and eventually ($\lozenge$).
The syntax of an \gls{scltl} formula is:
\begin{equation*}
    \varphi := \sigma \setor \lnot \sigma \setor \varphi \wedge \varphi \setor \varphi \vee \varphi  \setor \bigcirc \varphi \setor \varphi\ \mathcal{U}\ \varphi \setor \lozenge \varphi,
\end{equation*}
where $\sigma \in \Sigma$ and $\varphi$ is an \gls{scltl} formula. 

% First, for the case where the robot is tasked with leaving the building without going into the fire, our specification can be written as: $\lnot F \;\mathcal{U}\; O$ (translates to: ``not fire until outside'').
% Alternatively, if we want the robot to fight the fire, we have: $((\lnot F \;\mathcal{U}\; E) \land \lozenge F) \lor (\lnot F \; \mathcal{U}\; A)$ (``not fire until extinguisher, and eventually fire, or not fire until alarm''). This specification gives the robot the option of either using the extinguisher, or activating the sprinkler system to accomplish its task.

% To do so, we consider a sequence of truth assignments to the propositions, $\omega_A = \omega_0 \omega_1 \omega_2 \ldots$ where each $\omega_i \in 2^\Sigma$ contains the propositions that are true at that step, i.e. $\sigma \in \omega_i$ means that $\sigma$ is true at step $i$.

% We can evaluate the truth of a formula If the sequence of truth assignments makes the formula true, we say that it models the specification ($\omega \models \varphi)$.

To determine if a plan satisfies an \gls{scltl} specification, we need to consider the semantics of \gls{scltl} and the truth values of the propositions over time.
The semantics of an \gls{scltl} specification are defined over infinite words $\omega = \omega_0 \omega_1 \omega_2 \ldots$ with letters $\omega_i \in 2^\Sigma$.
% A trace $w = w_0 w_1 w_2 \ldots$ is a sequence of the truth values 
% At each time step $i$, a set of propositions $\omega_i \in 2^\Sigma$ are true and any proposition not in $\omega_i$ is false.
Intuitively, $\bigcirc \varphi$ is satisfied at step $i$ if $\varphi$ is satisfied at the next step ($i+1$). 
A formula $\varphi_1 \mathcal{U} \varphi_2$ is satisfied at step $i$ if $\varphi_1$ is satisfied at every step until $\varphi_2$ is satisfied.
A formula $\lozenge \varphi$ is satisfied at step $i$ if $\varphi$ is satisfied at some step $j > i$.
For the complete semantics of \gls{scltl}, refer to \citet{Kupferman2001}. \hkc{i am missing some forml statement about the fact that the truth value of scltl can be determined in finite traces}

Returning to our example of a robot putting out a fire in a burning building, we define the set of propositions $\Sigma = \{\texttt{fire}, \texttt{extinguisher}, \texttt{alarm}, \texttt{exit} \}$. \hkc{explain the physical grunding of these propositions. The main one that is confusing to me is "fire". I think you mean "fire" = an action of going to the location of the fire, rather than sensing fire.}
Using these propositions and the Boolean and temporal operators, we can specify tasks we want the robot to accomplish.
For example, if we want our fire-fighting robot to avoid fire until it either activates the alarm or finds the extinguisher and returns to put out the fire, we can write: $(\lnot \texttt{fire}\ \mathcal{U}\ \texttt{alarm}) \vee ((\lnot \texttt{fire}\ \mathcal{U}\ \texttt{extinguisher}) \wedge \lozenge \texttt{fire})$ (``not fire until alarm or not fire until extinguisher, and eventually fire'').
This formula is satisfied when the robot either does not visit any regions with fire and then visits the alarm or does not visit any regions with fire until it gets the extinguisher and then visits a region with fire.
% For example, if we want our fire-fighting robot to avoid regions with fire until it finds the extinguisher and then return to put out the fire, we can write: $(\lnot \texttt{fire}\ \mathcal{U}\ \texttt{extinguisher}) \wedge \lozenge \texttt{fire}$ (``not fire until extinguisher and eventually fire'')

% For example, if we want the robot to activate the alarm to put out the fire, we could write: $\lnot \texttt{fire} \mathcal{U} \texttt{alarm}$ (``not fire until alarm'').
% In order to satisfy this specification, the robot needs to avoid the fire until it reaches the alarm.
% Alternatively, if we want the robot to put out the fire using the fire extinguisher, we could write: $\lnot (\texttt{fire} \mathcal{U} \texttt{extinguisher}) \wedge \lozenge \texttt{fire}$ (``not fire until extinguisher and eventually fire'').
% In this case, the robot needs to avoid the fire until it finds the extinguisher and then go back to the fire.
% We could also give the robot the option of putting out the fire using either method: $(\lnot \texttt{fire}\ \mathcal{U}\ (\texttt{alarm})) \vee (\lnot (\texttt{fire}\ \mathcal{U}\ \texttt{extinguisher}) \wedge \lozenge (\texttt{fire})))$ (``not fire until alarm or not fire until extinguisher and eventually fire''). 
%We could also give the robot the option of putting out the fire using either method and then leaving the building: $(\lnot \texttt{fire} \mathcal{U} (\texttt{alarm} \wedge \texttt{outside})) \vee (\lnot (\texttt{fire} \mathcal{U} \texttt{extinguisher}) \wedge \lozenge (\texttt{fire}) \wedge \lozenge \texttt{outside}))$ (``not fire until alarm and eventually outside or not fire until extinguisher and eventually fire and eventually outside). 

% Note that \gls{scltl} formulae can be satisfied by finite words ($\omega_A^{fin} = \omega_0 \omega_1 \ldots \omega_n$) even though they have infinite time semantics. 
% This means that we are able to determine when a task has been successfully completed.
% For example, the specification  $\lnot F \;\mathcal{U}\; O$ (``not fire until outside'') is satisfied as soon as the robot reaches the outside of the building.
% means that $\varphi$ is satisfied at the next step by $\omega_{i+1}$, $\omega_i \models \varphi_1 \mathcal{U} \varphi_2$ means that $\varphi_1$ is satisfied at every step until $\varphi_2$ is satisfied by some $\omega_{j}$, and $\omega_i \models \lozenge \varphi$ means that $\varphi$ is satisfied by some $\omega_{j}$ with $j > i$.
% For the full semantics of \gls{scltl}, refer to \cite{}.


% Note that in \gls{scltl}, negation is only allow on individual propositions $\sigma$

% We define a complex task specification for our robot using \gls{scltl}.
% \gls{scltl} formulas are written over a set of atomic propositions $\Sigma$ where $\sigma \in \Sigma$ is a Boolean variable. 
% The syntax of \gls{scltl} is defined inductively as follows:
% \begin{equation*}
%     \varphi := \sigma \setor \lnot \sigma \setor \varphi \wedge \varphi \setor \varphi \vee \varphi  \setor \bigcirc \varphi \setor \varphi\ \mathcal{U}\ \varphi \setor \lozenge \varphi,
% \end{equation*}
% where $\sigma \in \Sigma$ and $\varphi$ is an \gls{scltl} formula. 
% The Boolean operators are negation ($\lnot$), conjunction ($\wedge$), and disjunction ($\vee$) and the temporal operators are next ($\bigcirc$), until ($\mathcal{U}$), and eventually ($\lozenge$). 
% An \gls{scltl} formula is how we communicate to the robot what its task is, and contains information on the ways it can accomplish that task.

% Consider, once again, a robot trapped in a burning building. We could imagine any number of specifications we would want our robot to satisfy. First, for the case where the robot is tasked with leaving the building without going into the fire, our specification can be written as: $\lnot F \;\mathcal{U}\; O$ (translates to: ``not fire until outside''). Alternatively, if we want the robot to fight the fire, we have: $((\lnot F \;\mathcal{U}\; E) \land \lozenge F) \lor (\lnot F \; \mathcal{U}\; S)$ (``not fire until extinguisher, and eventually fire, or not fire until sprinklers''). This specification gives the robot the option of either using the extinguisher, or activating the sprinkler system to accomplish its task.

% The semantics of \gls{scltl} are defined over infinite words in $2^\Sigma$. 
% Let word $\omega_A = \omega_0 \omega_1 \omega_2 \ldots$ where each element of the word $\omega_i \in 2^\Sigma$. 
% Intuitively, $w \models \bigcirc \varphi$ means that $\varphi$ is satisfied at the next step, $w \models \varphi_1 \mathcal{U} \varphi_2$ means that $\varphi_1$ is satisfied until $\varphi_2$ is satisfied in $w$, and $w \models \lozenge \varphi$ means that $\varphi$ is satisfied at some point in $w$.
% Note that \gls{scltl} formulas can be satisfied by finite words ($\omega_A^{fin} = \omega_0 \omega_1 \ldots \omega_n$) even though they have infinite time semantics. 
% This allows us to specify tasks that have a distinct end point, as opposed to one's which continue over an infinite time horizon.

\paragraph{Deterministic Finite Automaton}\label{sub:dfa-preliminaries}
%\glsresetall

%Because tasks specified in \gls{scltl} can be satisfied in finite time, 
% Intuitively, a \gls{dfa} contains a set of states $Z$ which the robot transitions between based on the letters in the word $\omega$.
A \gls{dfa} is constructed from an \gls{scltl} specification\footnote{We use Spot \cite{spot} to create the \gls{dfa} in our implementation.}, and can be used to determine if a word $w$ satisfies the specification.
% In order to determine what the robot must do in order to satisfy the specification, we transform the \gls{scltl} specification into a \gls{dfa} \cite{Kupferman2001}.
% When an accepting state in the \gls{dfa} is reached, the specification has been satisfied.
% Fig. \ref{fig:dfa_ts_pa}A contains the \gls{dfa} for the specification $(\lnot \texttt{fire}\ \mathcal{U}\ \texttt{alarm}) \vee (\lnot (\texttt{fire}\ \mathcal{U}\ \texttt{extinguisher}) \wedge \lozenge \texttt{fire})$.
Formally, a \gls{dfa} is a tuple $\mathcal{A}_{\varphi} = (Z, z_0, \Sigma, \delta_A, F)$. 
It contains a set of states, $Z$, with an initial state $z_0 \in Z$. 
% Transitions are made between states based on the truth values of propositions $\Sigma$ used to construct the specification $\varphi$.
The transition function $\delta_A: Z \times \Sigma \hkc{shouldn't this be $2^\Sigma ?$}\rightarrow Z$ takes in the current state, $z \in Z$ and the propositions $\sigma \in \Sigma$ \hkc{shouldn't this be $\Bar{\sigma} \in 2^\Sigma$?} that are true and returns the next state $z \in Z$ in the \gls{dfa}.
We \sout{also} define \sout{a set} $Z_{\text{next}}(z) = \{z' \in Z_{\text{next}}(z) \hkc{this does not make sense. do you mean z' $\in$ Z? }\ |\ \exists \sigma \in \Sigma \hkc{shouldn't this be $\Bar{\sigma} \in 2^\Sigma$?} \textrm{ s.t. } z'=\delta_A(z,\sigma) \hkc{shouldn't this be $(z,\Bar{\sigma} )$?}\}$ that contains the possible `next' \hkc{why have the ' ?} DFA states from the `current' DFA state.
The \gls{dfa} \sout{also contains} has a set of accepting states, $F \subseteq Z$, such that if \hkg{the execution of the DFA on a finite word $\omega=\Bar{\sigma}_1,\Bar{\sigma}_2,...,\Bar{\sigma}_n$ ends in }a state $z \in F$ \sout{is reached}, the \hkg{word belongs to the language of the DFA. Since the DFA is created from a \gls{scltl} specification, if the finite word is in the language, it means that the execution that created the word satisfies the specification.} \sout{specification is satisfied.}
A \gls{dfa} for the specification $(\lnot \texttt{fire} \mathcal{U} \texttt{extinguisher}) \wedge \lozenge \texttt{fire}$ is shown in Fig.~\ref{fig:defining-actions}.

%\adam{Depending on how clear the above is, we can remove this paragraph.}
%In the example show in Fig. \ref{fig:dfa_ts_pa}A, the robot starts in state $z_0$.
%The robot can either stay in this state via a ``self-transition'' or transition to another state.
%For state $z_0$, the self-transition is $\lnot \texttt{alarm} \wedge \lnot \texttt{extinguisher} \wedge \lnot \texttt{fire}$, meaning that as long as $\texttt{alarm}$, $\texttt{extinguisher}$, and $\texttt{fire}$ are false, the robot remains in $z_0$.
%Once the robot reaches the accepting state, $z_2$, we know the task has been accomplished.
%If the propositions the robot observed satisfy $\lnot \texttt{alarm} \wedge \texttt{extinguisher} \wedge \lnot \texttt{fire}$, meaning the robot finds the extinguisher without being in the fire or triggering the alarm, it transitions to state $z_1$.
% For this transition, the value of $\texttt{outside}$ could be either true or false.

% However, the \gls{dfa} only contains what the truth values of the abstract propositions need to be, and not neccessarily the value of the 

% In order to determine how a word might be relevant to the given task, \gls{dfa} can be constructed that accepts all words $\omega$ which satisfy an \gls{scltl} formula $\varphi$. 

% A \gls{dfa} is defined as a tuple $\mathcal{A}_{\varphi} = (Z, z_0, \Sigma, \delta_A, F)$ where:
% \begin{flushitemize}
% \item $Z$ is a finite set of states
% \item $z_0 \in Z$ is the initial state
% \item $\Sigma$ is the input alphabet
% \item $\delta_A : Z \times \Sigma \rightarrow Z$ is the transition function
% \item $F \subseteq Z$ is the set of accepting states
% \end{flushitemize}

% %For use later, we define the set $\Delta(z) = \{z' \ |\ \exists \sigma \in \Sigma\ \textrm{s.t.}\ z' = \delta(z,\sigma)\}$ of valid next states in the \gls{dfa} from state $z$.

% By constructing a \gls{dfa} from a given \gls{scltl} formula, we can track what an agent must do in order to accomplish its task.  A finite word $\omega_A^{fin} = \omega_0 \omega_1 \ldots \omega_n$ where $\omega_i \in \Sigma$ generates a finite trace $\tau_A^{fin} = z_0 z_1 \ldots z_{n+1}$ through a \gls{dfa} $\mathcal{A}$ where $z_{i+1} = \delta_A(z_i, \omega_i) \forall i = 0 ... n$.
% A trace $\tau_A^{fin}$ is an accepting trace if $z_n \in F$.

\paragraph{Labeled Transition System}\label{sub:ts-preliminaries}
% A \gls{lts} is used to abstract the physical environment of the robot.
% The \gls{dfa} contains an abstraction of the robot's task and does not consider geometric restrictions on the robot's motion.
% To take into account the physical environment the robot operates in, we use a \gls{lts}.
\hkc{might be better to start with this. and then logic and DFA, and then product automaton} \sout{The} \hkg{We use a} \gls{lts} \hkg{to} abstract the physical environment \hkg{of the robot.} \sout{into a set of states, each labeled with a set of propositions that are true in that state, and which states are physically connected.} \hkc{grammatically there are issues and it makes more sense to explain the abstraction after introducing the structure.}
Formally, LTS $\mathcal{T}$ is a tuple  $(X, x_0, \delta_T, w, \Sigma, l)$.
Here, $X$ is the current set of states with $x_0 \in X$ being the initial state of the robot.
The set of possible transitions between the states is given by $\delta_T \subseteq X \times X$, where a robot can move between two states $x_i, x_j$ if $(x_i, x_j) \in \delta_T$.
The weight $w: (x_i, x_j) \rightarrow \mathbb{R}^{+}$ is a cost incurred by making the transition $(x_i, x_j)$.
% Each state in the \gls{lts} has a set of propositions associated with it.
We use the labeling function $l: X \rightarrow 2^\Sigma$ to assign which propositions are true in state $x \in X$. 
The \gls{lts} for our problem represents a discretized map of the environment, where each cell \hkg{is an area of the workspace, the transitions are the connectivity of the space (which cells the robot can move between, and the labels}  contain information about the truth values of each proposition.
An example \gls{lts} is shown in Fig.~\ref{fig:defining-actions} where\hkg{, for example,}  $l(x_5)=\texttt{extinguisher}$ \hkg{and $l(x_4)=\emptyset$}.
% An abstraction of an environment is shown in Fig. \ref{fig:dfa_ts_pa}B.

% As the robot attempts to satisfy its specification and observes unknown space, it updates a map of its environment. We use this map to build a Weighted Finite Deterministic Transition System $\mathcal{T} = (S, s_0, \delta_T, w, \Sigma, l)$ where:
% \begin{flushitemize}
%     \item $S$ is a finite set of states
%     \item $s_0$ is the initial state
%     \item $\delta_T \subseteq S \times S$ is the set of transitions
%     \item $w: \xi \rightarrow \mathbb{R}^{+}$ assigns a weight to each transition
%     \item $\Sigma$ is a set of propositions
%     \item $l: S \rightarrow 2^\Sigma$ assigns a label to each state
% \end{flushitemize}

% A weighted transition system allows the agent to know what propositions are true or false in a particular area. We can define $\tau_T^{fin} = s_0 s_1 \ldots s_n$  as a finite trace through the transition system where $(s_i, s_{i+1}) \in \delta_T$.
% This trace generates a word $\omega_T^{fin} = l(s_0) l(s_1) \ldots l(s_n)$ which is the sequence of propositions that are visited by the robot during trace $\tau_T^{fin}$. So, for any path the robot travels in the known map, the transition system computes a word that represents how each step affects the boolean value of each proposition.


% \subsection{Deterministic Finite Automaton}\label{sub:dfa-preliminaries}
% \glsresetall

% %Because tasks specified in \gls{scltl} can be satisfied in finite time, 

% In order to determine how a word might be relevant to the given task, \gls{dfa} can be constructed that accepts all words $\omega$ which satisfy an \gls{scltl} formula $\varphi$. 

% A \gls{dfa} is defined as a tuple $\mathcal{A}_{\varphi} = (Z, z_0, \Sigma, \delta_A, F)$ where:
% \begin{flushitemize}
% \item $Z$ is a finite set of states
% \item $z_0 \in Z$ is the initial state
% \item $\Sigma$ is the input alphabet
% \item $\delta_A : Z \times \Sigma \rightarrow Z$ is the transition function
% \item $F \subseteq Z$ is the set of accepting states
% \end{flushitemize}

% %For use later, we define the set $\Delta(z) = \{z' \ |\ \exists \sigma \in \Sigma\ \textrm{s.t.}\ z' = \delta(z,\sigma)\}$ of valid next states in the \gls{dfa} from state $z$.

% By constructing a \gls{dfa} from a given \gls{scltl} formula, we can track what an agent must do in order to accomplish its task.  A finite word $\omega_A^{fin} = \omega_0 \omega_1 \ldots \omega_n$ where $\omega_i \in \Sigma$ generates a finite trace $\tau_A^{fin} = z_0 z_1 \ldots z_{n+1}$ through a \gls{dfa} $\mathcal{A}$ where $z_{i+1} = \delta_A(z_i, \omega_i) \forall i = 0 ... n$.
% A trace $\tau_A^{fin}$ is an accepting trace if $z_n \in F$.
% A finite run of $\mathcal{A}_\varphi$ is a sequence of states $x = x_0 x_1 \ldots x_n$ where $x_0 = z_0$, $\forall i \in \{1, \ldots n\}$ $x_i \in Z,$,  and $\forall i\; \exists \omega_i\subseteq\Sigma x_{i+1} = \delta_A(x_i, \omega_i) $. 
% A run is an accepting run if $x_n \in F$. 
% An input trace that realizes an accepting run is a $\varphi$-satisfying trace. 




% The semantics of \gls{scltl} are defined over infinite traces in $2^\Sigma$. Let $w = w_0 w_1 w_2 \ldots$, where $w_i \in 2^\Sigma$, be an infinite trace and $w^i = w_i w_{i+1} \ldots$, and $w_i = w_0 w_1 \ldots w_{i-1}$. Here $w_i$ is a finite prefix of $w$ \hkc{this is not good notation because there is an overloading of $w_i$ - does it mean the position i or the prefix up until, but not including, i? }. We denote that a sequence $w$ satisfies $\varphi$ by $w \models \varphi$. \sout{We let $w \models \varphi$ denote that trace $w$ satisfies formula $\varphi$.} The semantics are defined recursively as:

% \begin{flushitemize}
% \item $w \models \sigma\ if\ \sigma \in w_0$ \hkc{see comment above}
% \item $\lnot w \models \sigma\ if\ \sigma \notin w_0$
% \item $w \models \varphi_1 \vee \varphi_2\ if\ w \models \varphi_1\ or\ w \models \varphi_2$
% \item $w \models \varphi_1 \wedge \varphi_2\ if\ w \models \varphi_1\ and\ w \models \varphi_2$
% \item $w \models \bigcirc \varphi\ if\ w^1 \models \varphi$
% \item $w \models \varphi_1\ \mathcal{U}\ \varphi_2\ if\ \exists k \geq 0\ s.t.\ \varphi_2,\ and\ \forall i\in [0,k) \varphi^i \models \varphi_1$ \hkc{missing symbols}
% \item $w \models \lozenge \varphi\ if\ \exists k \geq 0\ s.t.\ w^k \models \varphi$
% \end{flushitemize}


% A \gls{dfa} can be constructed to determine if a word $\omega$ satisfies a \gls{csltl} specification.
% We can construct a \gls{dfa} to determine the words required to satisfy a \gls{scltl} specification.
% \adam{introduce language?}


% \begin{comment}
\paragraph{Product Automaton}

% We use the product automaton as a way to search for an accepting sequence of states to visit to satisfy a specification.
% \adam{Less confusing sentances - more lay robotics terms}
% A product automaton can be constructed that accepts all words that satisfy a specification and the associated traces required in the transition system to generate the words.
When the robot moves between states in the \gls{lts}, it \sout{builds} \hkg{creates} a word $\omega$ from the labels in each state. Using the \gls{dfa}, we can determine \sout{what} \hkg{which} transitions occur as a result of this word.
A \gls{pa} \sout{combines the two automata, in this case,} \hkg{captures the combined behavior of} the \gls{dfa} and \gls{lts}.
% Intuitively, transitions in the \gls{pa} are only allowed if they are allowed in both the \gls{dfa} and \gls{lts}.
\sout{This allows the physical environment to be combined with the abstraction of the \gls{scltl} specification.} \hkc{this is not accurate.} 
% As the robot moves through the environment, changing states in the \gls{wfdts}, it also moves between states in the \gls{dfa}.
% To keep track of this progression, plan, and determine when the specification is satisfied, we define a product automaton, which combines the task abstraction in the \gls{dfa} with the environment abstraction in the \gls{wfdts}.
% Intuitively, when the robot moves between states in the \gls{wfdts}, it causes the robot to move between states in the \gls{dfa} based up the \gls{wfdts} labels and the transition function of the \gls{dfa}.
Formally, $\mathcal{A}^P$ is a tuple $(P, p_0, \delta_P, w_P, F_p)$.
The product automaton states $P = X \times Z$ keep track of both the \gls{lts} state and the \gls{dfa} state, with $p_0 = (x_0, z_0)$ being the initial state.
A transition between states in the product automaton is possible only if \hkg{and only if} the transition is valid in both the \gls{lts} and \gls{dfa} and is defined by $\delta_P = \{(p_i, p_j) \ |\ (x_i, x_j) \in \delta_T, \delta_A(z_i, l(x_j\hkc{shouldn't this be $x_i$ ?})) = z_j\}$.
The weights on transitions in the \gls{pa} are the weights in the \gls{lts} ($w_P: P \times P \rightarrow \mathbb{R}^{+}$ s.t. $w_P(p_i, p_j) = w(x_i, x_j)$).
Similarly, the accepting states in the product automaton, $F_P$, are those states with accepting \gls{dfa} states ($F_P = X \times F$).
% Once we find a path through the product automaton to an accepting state, we can follow the sequence of states in the \gls{lts} to achieve that physically.

% In Fig. \ref{fig:dfa_ts_pa}C, a product automaton for the \gls{dfa} in Fig. \ref{fig:dfa_ts_pa}A and \gls{wfdts} in Fig. \ref{fig:dfa_ts_pa}B is shown.
% \end{comment}




% Given a \gls{dfa} $\mathcal{A}_\phi = (Z, z_0, \Sigma, \delta, F)$ and a transition system $\mathcal{T} = (S, s_0, \delta_T, w, \Sigma, l)$, we define a product automaton $\mathcal{A}^P = (P, p_0, \delta_P, w_P, F_p)$ where:
% \begin{flushitemize}
% \item $P = S \times Z$ is the finite set of states
% \item $p_0 = (s_0, z_0)$ is the initial state
% \item $\delta_P = \{(p_i, p_j) \ |\ (s_i, s_j) \in \delta_T, \delta_A(z_i, l(s_j)) = z_j\}$ is the set of transitions
% \item $w_P: P \times P \rightarrow \mathbb{R}^{+}$ is the weight function s.t. $w_P(p_i, p_j) = w(s_i, s_j)$
% \item $F_P = S \times F$ is the set of accepting states
% \end{flushitemize}

% A trace in the product automaton is defined as $\tau_P^{fin} = p_0 p_1 \ldots p_n$ where $(p_i, p_{i+1}) \in \delta_P$ is an accepting trace if $p_n \in F_P$.
% An accepting trace $\tau_P^{fin} = (s_0, z_0) (s_1, z_1) \ldots (s_n, z_n)$ defines an accepting trace in the \gls{dfa} $\mathcal{A}$, $\tau_A^{fin}$ which is generated by the word $\omega_A^{fin} = l(z_1) \ldots l(z_n)$ produced by the trace $\tau_T^{fin} = s_0 s_1 \ldots s_n$ in the transition system $\mathcal{T}$.

% The product automaton enables planning through a transition system (which is our labeled map), while simultaneously tracking what state in the \gls{dfa} the agent is in. This allows the agent to construct plans that move it through physical space, as well as the abstract task space defined by the \gls{dfa}.

%\subsection{Explaining how everything goes together}

% \subsection{LSP}

% Definition of a subgoal

==> related_work_pre_review.tex <==
\section{Related Works}
% \glsresetall

Temporal logic synthesis has been used to generate provably correct controllers, although predominantly in fully known environments \citep{Kress-Gazit2018, Fainekos2009, Bhatia2010, Lacerda2014, Smith2011}.
Recent work has begun to explore scenarios in which a task specified in \gls{ltl} needs to be completed in a partially explored environment \cite{Ayala2013temporal, Sarid2012guaranteeing, Lahijanian2016iterative}.
However, these works are more focused on satisfying the specification than minimizing cost.
\citet{Ayala2013temporal} introduce a method for a robot to explore an environment while not violating an \gls{scltl} specification until it has found a path to satisfy the specification.
This method uses a heuristic based on the specification and known space to decide where to travel next.
However, it does not incorporate information about what could be in unknown space to minimize the cost of fulfilling the specification, resulting in suboptimal plans in general.
\citet{Sarid2012guaranteeing} explore an environment while satisfying a specification and, as more of the environment is revealed, replan to incorporate newly discovered areas into the specification, though the cost of satisfying the specification is not considered.
In \citet{Lahijanian2016iterative}, given a specification and a map of an environment, the authors plan a path to satisfy the specification and replan when they encounter unexpected obstacles.
Again, this work does not consider potential cost related to unknown obstacles, but incorporates it as obstacles are encountered.

To minimize the cost of satisfying \gls{ltl} specifications, other recent works have used learning based approaches \cite{littman2017ltl, Fu2015probably, li2017reinforcement, li2019formal, teaching_multiple}.
\citet{littman2017ltl} demonstrate a formalism for building a \gls{mdp} from an \gls{ltl} specification that enables Q-learning to provably converge.
\citet{teaching_multiple} present a method for decomposing an \gls{ltl} specification into subtasks, which can then be learned using separate Deep Q-networks and combined in new specifications. 
However, each of these methods have been limited to relatively small, fully observable grid worlds.
\citet{li2017reinforcement} demonstrate learning in continuous manipulation environments, but are similarly restricted to fully observable domains.
\citet{sadigh2014learning} and \citet{Fu2015probably} apply learning to unknown environments and learn the transition matrices for \acrshort{mdp}s built from \gls{ltl} specifications.
However, these learned models do not generalize to new specifications and are demonstrated on relatively small grid worlds.
\citet{paxton2017combining} introduce uncertainty into their problem by allowing their world to evolve in a manner unknown to the autonomous agent.
The agent is given a feature vector of the current state and learns a transition matrix for a small set of discrete actions in a driving domain.
However, the authors limit their planning horizon to 10 seconds, which is insufficient for the kinds of task specifications explored in this paper.
Moreover, though such systems can be augmented to ensure safety \citep{li2019formal}, in reinforcement learning it is difficult to guarantee that a given specification will not be violated. 
%\citet{Stein2018} introduce an abstraction that allows a robot to plan over long time horizons in partially explored environments while completing a task in minimum time.
%However, their abstraction only allows for goal directed navigation tasks.

% \paragraph{Planning with Linear Temporal Logic in Unknown Environments}
% Temporal logic synthesis has been successfully used in many robot applications to generate provably correct control in fully known environments. \citep{Kress-Gazit2018, Fainekos2009, Lacerda2014, Bhatia2010, Smith2011}.
% % However, robots often need to operate in partially known environments.
% However, as robots often do not have full knowledge of their environments, work has begun to explore scenarios in which robots attempt to satisfy specifications in partially unknown environments \citep{Ayala2013temporal, Sarid2012guaranteeing, Lahijanian2016iterative}.
% While these works guarantee a robot will either fully accomplish a specification or accomplish as much as it is able to, they do not consider the time it takes to satisfy the specification.
% In \citet{Ayala2013temporal}, given a specification, the authors explore the environment while not violating the specification until they can find a path to satisfy the specification.
% In \citet{Sarid2012guaranteeing}, the authors explore an environment while satisfying a specification and as more of the environment is revealed, add these tasks to the specification.
% In \citet{Lahijanian2016iterative}, given a specification and a map of an environment, the authors plan a path to satisfy the specification and replan when they encounter unexpected obstacles.

% \paragraph{Learning to Satisfy Linear Temporal Logic Specifications}
% As mentioned previously a number of approaches use learning to try to find an optimal plan.  Because \gls{ltl} tasks are non-markovian in nature, traditional reinforcement learning approaches can fail to converge if the state is not augmented in some way. \citet{littman2017ltl} demonstrate a formalism for building an \gls{mdp} from an \gls{ltl} specification that enables Q-learning to provably converge. \citet{sadigh2014learning} and \citet{Fu2015probably} learn the transition matrices for \acrshort{mdp}'s built from \gls{ltl} specifications, but do not generalize their learned models to new specifications. In more recent work, \citet{teaching_multiple} present a method for decomposing an \gls{ltl} specification into subtasks, which can then be learned using separate Deep Q-networks and combined differently depending on the specification. Unfortunately, each of these methods have been limited to relatively small, fully observable grid worlds \citep{teaching_multiple, sadigh2014learning, Fu2015probably, littman2017ltl}. \citet{li2017reinforcement} demonstrate learning in continuous environments for task and motion planning, but are similarly restricted to fully observable domains.  \citet{paxton2017combining} introduce uncertainty into their problem by allowing their world to evolve in a manner unknown to the autonomous agent. The robot is given a feature vector of the current state and learns a transition matrix for a small set of discrete actions in a driving domain. However, the authors limit their planning horizon to 10 seconds, and do not plan directly from sensor input from the environment. Using reinforcement learning for these tasks in the presence of uncertainty it difficult for large problems due to the amount of data require for training. Moreover, though such systems can be augmented to ensure safely \citep{li2019formal}, reinforcement learning in general cannot guarantee that a given specification will not be violated.

%\paragraph{Learned Subgoal Planning}
%For goal-directed navigation tasks, \citep{Stein2018} makes progress in planning to minimize cost in partially explored environments. To make tractable predictions about the unknown portion of the environment, \citep{Stein2018} factors the Bellman Equation to evaluate expected cost of an action in terms of the high-level decisions available to an agent, and the high-level outcomes that result. Specifically, they define subgoals in the plans they generate as \emph{frontiers}---the boundaries between free and unknown space---and consider attempting to reach the final goal beyond each of these frontiers as a separate high-level action. By reformulating the equations for planning in terms of these high-level actions---for which they learn the costs and probabilities of success---and outcomes, the agent can navigate intelligently in partially revealed environments without the need to enumerate all possible configurations of unknown space. However, in \cite{Stein2018}, the authors focus on the task of goal-directed navigation only. As a result, the only outcomes the system considers when choosing a particular high-level action are whether the frontier of interest will or will not lead to the unseen goal. For more complex tasks, single goal locations no longer make sense---the fire extinguisher may be in the opposite direction of the fire---and planning intelligently to achieve specifications with such non-markovian goals requires considering less simplistic high-level actions and outcomes. We build on the principles of \cite{Stein2018}---using supervised learning to learn high level outcomes of actions through unknown space---and apply them to our new abstraction which encapsulates the intricacies of non-markovian tasks.

% To estimate cost of traveling through one subgoal, they train a neural network to predict three properties of the unknown space beyond the associated frontier. First, the network estimates the probability of the goal being beyond a frontier. Then the network predicts the cost associated with travelling to the goal (if possible), and the cost of attempting to travel to the goal, failing to do so, and returning to known space. Using these three estimated properties, the agent finds the optimal action by considering different ordering of subgoals (i.e., try to reach the goal through this door first, then down the hall, or vice-versa).




==> theory_backup.tex <==
\section{Planning in unknown environments with co-safe LTL specifications}
\label{sec:planning-old}

% \begin{flushitemize}
% \item Plan for minimum cost in partially known enviornments
% \begin{itemize}
%     \item What to do in known space and unknown space
%     \item could use POMDP, but intractable
%     \item Inspired by LSP and Automata base planning
% \end{itemize}
% \item What an action is
% \item Planning in known environment with product automaton - graph search
% \item Define actions allow us to estimate the cost of choosing a particular frontier and the way to get there - $a_{f,z,z'}$ and what the robot attempts to accomplish beyond that frontier
% \begin{itemize}
%     \item An action either succeeds or fails
%     \item test
% \end{itemize}
% \end{flushitemize}

Our objective is to minimize the total expected cost while satisfying a \gls{scltl} specification in partially explored environments. As mentioned previously, planning under uncertainty can be modeled as a \gls{pomdp}, and within this framework, the expected cost of taking the optimal action can be computed using a belief-space variant of the Bellman equation (todo: cite):


\begin{equation}\label{eq:base-eq-old}
Q(b_t, a_t \in \mathcal{A}(b_t)) = \sum_{b_{t+1}} P(b_{t+1} | b_t, a_t)\left[ R(b_{t+1}, b_{t}, a_t) + \min_{a_{t+1}\in \mathcal{A}(b_{t+1})} Q(b_{t+1}, a_{t+1}) \right]
\end{equation}

%This calculation requires considering the full distribution over environments, including all possible configurations of unknown space, and so is intractable in general for large problems. A key insight from \citet{Stein2018} however, is that we can greatly reduce the complexity of this computation by identifying a small number of discreet, \emph{high-level} actions which fully encompass the different ways a robot can attempt to accomplish its task. Then, by splitting future beliefs in to two classes---futures where the chosen action succeeds and futures where it fails---we can simply solve for the ordering of actions which 

Solving this equation for the optimal action requires considering the full distribution over environments, including all possible configurations of unknown space, and so is intractable in general for large problems. We can simplify the problem however, by planning with subgoals, as in \cite{Stein2018}. For goal-directed navigation, \citet{Stein2018} define a subgoal as traveling to a particular \emph{frontier}---a contiguous boundaries between free and unknown space---and attempting to reach the final goal beyond that frontier. The key insight from \cite{Stein2018}, is that we can greatly reduce the complexity of computing the optimal action by identifying a set of discreet, \emph{high-level} actions, and splitting future beliefs in to two classes---futures where taking a given action causes the robot to complete its task, and futures where it does not. For more complex tasks however, exploring beyond a single frontier to complete a task may no longer make sense (e.g., the fire extinguisher may be in the opposite direction of the fire). Thus, in this work, we consider a new set of actions, and a new way to divide future belief states in order to plan to satisfy \gls{scltl} specifications. To enable intelligent planning for more complex tasks, specified by co-safe LTL, we require a richer action representation, one in which we can reason about the different ways an agent might make progress towards satisfying the task specification. For each high-level action, we must also estimate a likelihood that these actions will succeed in making progress while navigating through unknown space, as well as the ``instantaneous cost’' of each action, conditioned on whether it succeeds or fails. Sec 4.1 is devoted to formally defining our high-level actions, the possible outcomes of executing an action, and the expected instantaneous cost of each.


%We introduce \textit{high-level actions} as an abstraction to allow the agent to plan while taking into its behavior in both known and unknown space.
% These high-level actions encompass what the agent should do in known space and what it can attempt to accomplish in unknown space.
%We can then use a variant of \gls{mcts} to find the optimal action that will minimize the cost of satisfying a \gls{scltl} specification.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/LTL_define_actions.png}
    \caption{\textbf{Schematic showing the high-level actions for a simple environment.} In our formulation, the boundaries between free and unknown space (\emph{frontiers}) and the states in the \acrfull{dfa} define the high-level actions available to an agent. Full details of how we use these high-level actions to plan are given in Sec.~\ref{sec:planning}. \adam{can we change the numbering on the dfa states so that 0 is the init state in the final figure? Not really a big deal, but could result in less confusion to unfamiliar readers.}}
    \label{fig:defining-actions}
\end{figure}

\subsection{Defining our Action Set}
\label{sec:sub-action-set-old}

We require a set of actions which fully encompasses the different ways a robot can make progress in completing a given task, and which allow us to define useful groupings of future beliefs after an action is taken. As discussed in Sec. \ref{sub:dfa-preliminaries}, the \gls{dfa} defined by a given task specification is a useful model for tracking an agent's progress toward completing that task. In order to reach an accepting state and satisfy its specification, our robot must take actions that cause it to transition to new states in the \gls{dfa}. For example, if our agent needs to activate the sprinklers to put out the fire, each sprinkler control panel we have observed corresponds to a way the agent could advance its state in the \gls{dfa} and make progress in its task. In our problem setting, the map is only partially revealed at the outset, and the agent must consider that there may be extinguishers and alarms and fires that have not yet been discovered. 

%Our goal is to minimize the expected cost of satisfying a specification in such partially explored environments and, as such, model our planning task as a \gls{pomdp}. Within this framework, the expected cost of taking the optimal action can be computed using the Bellman equation, yet requires considering the distribution over environments, including all possible configurations of unknown space. Though this computation is intractable in general, we build on a key insight from \citet{Stein2018}: if we define useful high-level actions and can simplify the space of possible outcomes to only ``success'' or ``failure'' to transition in the \gls{dfa}, we can greatly reduce the branching factor and therefore the computational cost of planning.

%As discussed in Sec. \ref{sub:dfa-preliminaries}, the \gls{dfa} defined by a given task specification is a useful model for tracking an agent's progress toward completing that task. In order to reach an accepting state and satisfy its specification, our robot must take actions that cause it to transition to new states in the \gls{dfa}. For example, if our agent needs to activate the sprinklers to put out the fire, each sprinkler control panel we have observed corresponds to a way the agent could advance its state in the \gls{dfa} and make progress in its task. In our problem setting, the map is only partially revealed at the outset, and the agent must consider that there may be extinguishers and alarms and fires that have not yet been discovered. Our goal is to minimize the expected cost of satisfying a specification in such partially explored environments and, as such, model our planning task as a \gls{pomdp}. Within this framework, the expected cost of taking the optimal action can be computed using the Bellman equation, yet requires considering the distribution over environments, including all possible configurations of unknown space. Though this computation is intractable in general, we build on a key insight from \citet{Stein2018}: if we define useful high-level actions and can simplify the space of possible outcomes to only ``success'' or ``failure'' to transition in the \gls{dfa}, we can greatly reduce the branching factor and therefore the computational cost of planning.


Inspired by \cite{Stein2018}, the action set is partially defined by \emph{frontiers}---contiguous boundaries between free and unknown space. Specifically, the robot first plans through $\mathcal{A}^P$ in known space to a point along a frontier and then enters the unknown space beyond that subgoal to attempt to transition to a new state in the \gls{dfa}. For example, if turning on the alarm is relevant to the robot's task, the agent might choose any of the frontiers in the map and travel through that frontier with the intent of finding and activating an alarm (all while avoiding the fire). If the robot does not transition in the \gls{dfa}, the action is said to fail; transitioning to the new \gls{dfa} state defines a successful action. As the robot explores and observes new space, it will invariably find that it can plan to advance its state in the \gls{dfa} within space it has revealed. The set of high-level actions available to the agent therefore must also include actions in which the agent progresses in the \gls{dfa} in known space (by computing the optimal trajectory to satisfy this portion of the specification) and then navigates to a frontier in pursuit of further transitions. For our firefighting example, if the robot has revealed a fire extinguisher, attempting to find the fire beyond a particular frontier and picking up the observed extinguisher along the way is considered a single high-level action. Fig.~\ref{fig:defining-actions} shows the high-level actions for a simple example.
%Therefore, if there were arbitrarily many extinguishers, only the lowest cost path to a given frontier that includes collecting the extinguisher would be added to the action set.
High-level actions are completely described by the tuple: $a_{f, z, z'} = (f, z, z')$, where $f$ is the frontier of interest, $z$ is the state in the \gls{dfa} after traveling through the product automaton to the frontier in known space, and $z'$ is the state the agent would attempt to reach beyond the frontier.
As in \cite{Stein2018}, we also check if the task can be satisfied completely in known space, and add that action to our set of subgoals.



\subsection{Planning with Subgoals}

Consider a robot at position $p$ in the product automaton, attempting to plan to reach an accepting state. We define a policy $\Pi$ as a binary tree of subgoals, where each subgoal has some probability of successfully transitioning to its desired state in the \gls{dfa}, a cost associated with making that transition, and a cost of attempting to transition, and failing. Because each action is not deterministic, in order to find the optimal policy, after selecting a subgoal, the robot must choose the next subgoal both for the case where that action succeeds---the robot transitions to the desired state in the \gls{dfa}---and when it fails.

One branch of this policy tree consists of a history $\hist = \{a_0, o_0, a_1, o_1, ... \}$ of actions $a_{f, z, z'} \in \mathcal{A}(b_\hist$), and outcomes, $o \in \{1, 0\}$ (success or failure). During a planning rollout, the agent imagines that some information about the environment is revealed as it executes exploratory actions. If the agent fails to transition to state $z'$ after imagining execution of $a_{f, z, z'}$ ($o=0$), this exploratory action is removed from its action set for the remainder of the rollout, since the frontier $f$ is then known not to allow this transition. By contrast, if the action succeeds ($o=1$), the action is guaranteed to succeed again, equivalent to setting the success probability of action $a_{f, z, z'}$ to 1; updating the action's success probability records that the agent has successfully transitioned from $z$ to $z'$ via frontier $f$ and that it could do so again if it were necessary. At each decision in the policy tree, the tuple $\{\mathcal{A}^p, p_r, \hist\}$, which encapsulates the product automaton $\mathcal{A}^p$, the robot's current state in $\mathcal{A}^p$, $p_r$, and the history of actions and outcomes, $\hist$, is a sufficient statistic for the belief, $b_\hist$.

The cost of choosing subgoal $a_{f, z, z'}$ from belief $b_\hist$, then following the optimal policy $\Pi$ is given below:

\begin{equation}\label{eq:ltl-subgoal-planning-equation}
  \begin{split}
  Q(b_t, a_{s,z,z'}) = & \sum_{b_{t+1}} P(b_{t+1}|b_t, a_{f,z,z'})\left(R(b_\hist, a_{s,z,z'}, z_{t+1}) + \min_{a' \in \mathcal{A}(b_{t+1})} Q(\{p_r, z_{t+1}\}, a') \right)
  \end{split}
\end{equation}


==> theory_copy.tex <==
\begin{comment}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{figures/alternative_approaches.png}
\caption{Placeholder for schematic of our approach, possibly comparing with alternative approaches
% Possible approaches to find a minimum cost path in a partially unknown environment. Given a specifcation with several frontiers, the robot can greedily only consider the next step and try to transition to a next state in the \gls{dfa}, hypothesize all possible propositions it may encounter behind the frontiers in all orders, or minimize the cost to follow a single trace through the \gls{dfa}. %\noteitem{Chris: I don't think we're going with the trace based approach anymore. Adam: sounds good, I think a figure showing something like this will still be useful if we can make it not messy and we will remove the trace part,}
}
\label{fig:alternatives}
\end{figure}
\end{comment}

\section{Planning with co-safe LTL Specifications}
\label{sec:planning}

Our objective is to minimize the total expected cost while satisfying a \gls{scltl} specification in partially explored environments. As mentioned previously, planning under uncertainty can be modeled as a \gls{pomdp}, and within this framework, the expected cost of taking the optimal action can be computed using the Bellman equation:

\begin{equation}\label{eq:base-eq}
Q(b_t, a_t \in \mathcal{A}(b_t)) = \sum_{b_{t+1}} P(b_{t+1} | b_t, a_t)\left[ R(b_{t+1}, b_{t}, a_t) + \min_{a_{t+1}\in \mathcal{A}(b_{t+1})} Q(b_{t+1}, a_{t+1}) \right]
\end{equation}

%This calculation requires considering the full distribution over environments, including all possible configurations of unknown space, and so is intractable in general for large problems. A key insight from \citet{Stein2018} however, is that we can greatly reduce the complexity of this computation by identifying a small number of discreet, \emph{high-level} actions which fully encompass the different ways a robot can attempt to accomplish its task. Then, by splitting future beliefs in to two classes---futures where the chosen action succeeds and futures where it fails---we can simply solve for the ordering of actions which 

Solving this equation for the optimal action requires considering the full distribution over environments, including all possible configurations of unknown space, and so is intractable in general for large problems. We can simplify the problem however, by planning with subgoals, as in \cite{Stein2018}. For goal-directed navigation, \citet{Stein2018} define a subgoal as traveling to a particular \emph{frontier}---a contiguous boundaries between free and unknown space---and attempting to reach the final goal beyond that frontier. The key insight from \cite{Stein2018}, is that we can greatly reduce the complexity of computing the optimal action by identifying a set of discreet, \emph{high-level} actions, and splitting future beliefs in to two classes---futures where taking a given action causes the robot to complete its task, and futures where it does not. For more complex tasks however, exploring beyond a single frontier to complete a task may no longer make sense (e.g., the fire extinguisher may be in the opposite direction of the fire). Thus, in this work, we consider a new set of actions, and a new way to divide future belief states in order to plan to satisfy \gls{scltl} specifications.  This section is devoted to a discussion of the theoretical foundations of our work. 

%As discussed in Sec. \ref{sub:dfa-preliminaries}, the \gls{dfa} defined by a given task specification is a useful model for tracking an agent's progress toward completing that task. In order to reach an accepting state and satisfy its specification, our robot must take actions that cause it to transition to new states in the \gls{dfa}. For example, if our agent needs to activate the sprinklers to put out the fire, each sprinkler control panel we have observed corresponds to a way the agent could advance its state in the \gls{dfa} and make progress in its task.

%propose a novel abstraction, in which the high-level actions are derived from the given task, as well as subgoals defined by \emph{frontiers} in the robot's map as in \cite{Stein2018}. The planner selects a high-level action by computing expected cost with Monte-Carlo Tree Search, which relies on the output of a convolutional neural network to estimate (1) the transition probabilities and (2) costs of making transitions through unknown space, both needed to inform planning decisions. This section is devoted to a discussion of the theoretical foundations of our work. 

%\begin{equation}\label{eq:factored-bellman}
%\begin{split}
%Q(b_t, a_t \in \mathcal{A}(b_t)) = P_S(b_{t+1}\in G|b_t, a_t)\sum_{b_{t+1} \in G} P_G(b_{t+1} | b_t, a_t) \left[ R(b_{t+1}, b_{t}, a_t) + \!\!\!\!\!\min_{a\in \mathcal{A}(b_{t+1})}\!\!\!\!\! Q(b_{t+1}, a) \right]\\
%(1-P_S(b_{t+1}\in G | b_t, a_t))\sum_{b_{t+1} \not\in G} P_{\bar{G}}(b_{t+1} | b_t, a_t) \left[ R(b_{t+1}, b_{t}, a_t) + \!\!\!\!\!\min_{a\in \mathcal{A}(b_{t+1})}\!\!\!\!\! Q(b_{t+1}, a) \right],
%\end{split}
%\end{equation}

%To that end, we propose an abstract representation of a given task which defines subgoals as the \emph{high-level actions} relevant for solving that task in a particular environment. In our abstraction, the high-level actions are derived from the product automaton, as well as the \emph{frontiers} in the robot's map as in \cite{Stein2018}. The planner selects a high-level action by computing expected cost with Monte-Carlo Tree Search, which relies on the output of a convolutional neural network to estimate (1) the transition probabilities and (2) costs of making transitions through unknown space, both needed to inform planning decisions. This section is devoted to a discussion of the theoretical foundations of our work.


\begin{comment}
\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{figures/dfa_until_eventually_example.png}
\caption{left: $\lnot a \mathcal{U} b$ right: $\lnot a \wedge \lozenge b$}\label{fig:dfa_eventually_until_example}
\end{figure}
\end{comment}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/LTL_define_actions.png}
    \caption{\textbf{Schematic showing the high-level actions for a simple environment.} In our formulation, the boundaries between free and unknown space (\emph{frontiers}) and the states in the \acrfull{dfa} define the high-level actions available to an agent. Full details of how we use these high-level actions to plan are given in Sec.~\ref{sec:planning}.}
    \label{fig:defining-actions}
\end{figure}

%One thing to note is that there is no mention of cost anywhere in these specifications, meaning we can take a wrong turn and still recover to satisfy our assignment. It is up to our planner to find paths that satisfy the task in finite time as quickly as possible. LTL specifications that can be proven to have one or more accepting states that can be reached in finite time are classified as syntactically co-safe LTL. We will restrict our study to those types of specifications.

%\subsection{Translating a Specification}
%\label{sub:translating}
%\adam{Move parts to preliminaries as necessary}

%\chris{I've moved over a lot of this stuff. might be a good idea to delete.}


\begin{comment}
\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{figures/fire_extinguisher_control.png}
\caption{This Directed Finite Automaton represents the states and transitions of the following LTL specification: $((\lnot F \mathcal{U} E) \land \lozenge F) \lor (\lnot F \mathcal{U} S)$, where F stands for fire, E for extinguisher, and S for the sprinkler control room.  State 1 represents the only accepting state which satisfies the specification, while state 3 is only reached if the specification fails. We can reduce the complexity of this automaton by realizing we never are interested in planning to state 3. Moreover, the probability of reaching both the fire and the extinguisher at the same time is essentially zero. As such there are three viable traces of this \gls{dfa} that go from the initial state 2 to accepting state 1.}\label{fig:Automata}
\end{figure}
\end{comment}

%As presented by Li et al. \cite{Li2013}, transitions in an Automaton defined by an LTL specification can be represented by a conjunction of atomic propositions and negations of propositions. If we know the propositions that may exist in our environment, we can write any transition as two n-dimensional vectors, where n represents the number of propositions of interest. This representation, which will be presented in detail in section \ref{sub:encoding}, allows us to input the transitions of our automaton to the network, thereby enabling it to predict the transition probabilities and costs of any subgoal from the robot's action set. For notational purposes, a transition can be written as a tuple of the original state in the \gls{dfa}, and the state reached after the transition: $t = (z, z')$

%\section{Computing Cost}
%\label{sec:computing-cost}

\subsection{Defining our Action Set}
\label{sec:sub-action-set}

We require a set of actions which fully encompasses the different ways a robot can make progress in completing a given task, and which allow us to define useful groupings of future beliefs after an action is taken. As discussed in Sec. \ref{sub:dfa-preliminaries}, the \gls{dfa} defined by a given task specification is a useful model for tracking an agent's progress toward completing that task. In order to reach an accepting state and satisfy its specification, our robot must take actions that cause it to transition to new states in the \gls{dfa}. For example, if our agent needs to activate the sprinklers to put out the fire, each sprinkler control panel we have observed corresponds to a way the agent could advance its state in the \gls{dfa} and make progress in its task. In our problem setting, the map is only partially revealed at the outset, and the agent must consider that there may be extinguishers and alarms and fires that have not yet been discovered. 

%Our goal is to minimize the expected cost of satisfying a specification in such partially explored environments and, as such, model our planning task as a \gls{pomdp}. Within this framework, the expected cost of taking the optimal action can be computed using the Bellman equation, yet requires considering the distribution over environments, including all possible configurations of unknown space. Though this computation is intractable in general, we build on a key insight from \citet{Stein2018}: if we define useful high-level actions and can simplify the space of possible outcomes to only ``success'' or ``failure'' to transition in the \gls{dfa}, we can greatly reduce the branching factor and therefore the computational cost of planning.

%As discussed in Sec. \ref{sub:dfa-preliminaries}, the \gls{dfa} defined by a given task specification is a useful model for tracking an agent's progress toward completing that task. In order to reach an accepting state and satisfy its specification, our robot must take actions that cause it to transition to new states in the \gls{dfa}. For example, if our agent needs to activate the sprinklers to put out the fire, each sprinkler control panel we have observed corresponds to a way the agent could advance its state in the \gls{dfa} and make progress in its task. In our problem setting, the map is only partially revealed at the outset, and the agent must consider that there may be extinguishers and alarms and fires that have not yet been discovered. Our goal is to minimize the expected cost of satisfying a specification in such partially explored environments and, as such, model our planning task as a \gls{pomdp}. Within this framework, the expected cost of taking the optimal action can be computed using the Bellman equation, yet requires considering the distribution over environments, including all possible configurations of unknown space. Though this computation is intractable in general, we build on a key insight from \citet{Stein2018}: if we define useful high-level actions and can simplify the space of possible outcomes to only ``success'' or ``failure'' to transition in the \gls{dfa}, we can greatly reduce the branching factor and therefore the computational cost of planning.


Inspired by \cite{Stein2018}, the action set is partially defined by \emph{frontiers}---contiguous boundaries between free and unknown space. Specifically, the robot first plans through $\mathcal{A}^P$ in known space to a point along a frontier and then enters the unknown space beyond that subgoal to attempt to transition to a new state in the \gls{dfa}. For example, if turning on the alarm is relevant to the robot's task, the agent might choose any of the frontiers in the map and travel through that frontier with the intent of finding and activating an alarm (all while avoiding the fire). If the robot does not transition in the \gls{dfa}, the action is said to fail; transitioning to the new \gls{dfa} state defines a successful action. As the robot explores and observes new space, it will invariably find that it can plan to advance its state in the \gls{dfa} within space it has revealed. The set of high-level actions available to the agent therefore must also include actions in which the agent progresses in the \gls{dfa} in known space (by computing the optimal trajectory to satisfy this portion of the specification) and then navigates to a frontier in pursuit of further transitions. For our firefighting example, if the robot has revealed a fire extinguisher, attempting to find the fire beyond a particular frontier and picking up the observed extinguisher along the way is considered a single high-level action. Fig.~\ref{fig:defining-actions} shows the high-level actions for a simple example.
%Therefore, if there were arbitrarily many extinguishers, only the lowest cost path to a given frontier that includes collecting the extinguisher would be added to the action set.
High-level actions are completely described by the tuple: $a_{f, z, z'} = (f, z, z')$, where $f$ is the frontier of interest, $z$ is the state in the \gls{dfa} after traveling through the product automaton to the frontier in known space, and $z'$ is the state the agent would attempt to reach beyond the frontier.
As in \cite{Stein2018}, we also check if the task can be satisfied completely in known space, and add that action to our set of subgoals.

% However, because there may be arbitrarily many of a particular proposition in the robot's map, it may be impractical to consider planning to each as distinct action. In order to reduce the branching factor in a plan while maintaining optimality\todo{This is true, but unclear. You need to make clear \emph{why} this is necessary for maintaining optimality. This part of Sec 4.1 is the only bit where I still have clarity issues. The example *after* this bit isn't enough to resolve the confusion once it exists.}, we consider the action of planning through a frontier to include any transitions the robot makes along the way. Continuing our example, if the robot has revealed a fire extinguisher, attempting to find the fire beyond a particular frontier, while picking up the extinguisher along the way is considered a single high-level action. Therefore, if there were arbitrarily many extinguishers, only the lowest cost path to a given frontier that includes collecting the extinguisher would be added to the action set. Thus, high-level actions are completely described by the tuple: $a_{f, z, z'} = (f, z, z')$, where $f$ is the frontier of interest, $z$ is the state in the \gls{dfa} after traveling through the product automaton to the frontier in known space, and $z'$ is the state the agent would attempt to reach beyond the frontier. As in \cite{Stein2018}, we also check if the task can be satisfied completely in known space, and add that action to our set of subgoals.


\subsection{Planning with Subgoals}

Consider a robot at position $p$ in the product automaton, attempting to plan to reach an accepting state. We define a policy $\Pi$ as a binary tree of subgoals, where each subgoal has some probability of successfully transitioning to its desired state in the \gls{dfa}, a cost associated with making that transition, and a cost of attempting to transition, and failing. Because each action is not deterministic, in order to find the optimal policy, after selecting a subgoal, the robot must choose the next subgoal both for the case where that action succeeds---the robot transitions to the desired state in the \gls{dfa}---and when it fails.

One branch of this policy tree consists of a history $\hist = \{a_0, o_0, a_1, o_1, ... \}$ of actions $a_{f, z, t} \in \mathcal{A}(b_\hist$), and outcomes, $o \in \{1, 0\}$ (success or failure). During a planning rollout, the agent imagines that some information about the environment is revealed as it executes exploratory actions. If the agent fails to transition to state $z'$ after imagining execution of $a_{f, z, z'}$ ($o=0$), this exploratory action is removed from its action set for the remainder of the rollout, since the frontier $f$ is then known not to allow this transition. By contrast, if the action succeeds ($o=1$), the action is guaranteed to succeed again, equivalent to setting the success probability of action $a_{f, z, z'}$ to 1; updating the action's success probability records that the agent has successfully transitioned from $z$ to $z'$ via frontier $f$ and that it could do so again if it were necessary. At each decision in the policy tree, the tuple $\{\mathcal{A}^p, p_r, \hist\}$, which encapsulates the product automaton $\mathcal{A}^p$, the robot's current state in $\mathcal{A}^p$, $p_r$, and the history of actions and outcomes, $\hist$, is a sufficient statistic for the belief, $b_\hist$.

%The actions available to the agent from a given state in the product automaton depend on the actions already considered in that history. For example, if the robot has already considered trying and failing to find the exit down a particular path, it should not try again\todo{This is not very clear to people who aren't us. Might want to talk about how our observations update some underlying (abstract) state of the map and \emph{then} how that change in the map translates to updated set of actions later on (both with new probability-1 actions and probability-0 actions).}. 

The cost of choosing subgoal $a_{f, z, z'}$ from belief $b_\hist$, then following the optimal policy $\Pi$ is given below:

 \begin{equation}\label{eq:ltl-subgoal-planning-equation}
  \begin{split}
  Q(b_\hist, a_{f,z,z'}) = & \underbrace{D(p_r, p_f)}_{1.} +
  \underbrace{P_S(o(a) = 1|b_\hist, a)}_{2.} \times
  \left[\underbrace{R_S(b_\hist,a)}_{3.} + \min_{a' \in \mathcal{A}(b_{\hist a o})} \underbrace{Q(\{\mathcal{A}^p, p_a, \hist a o\}, a')}_{4.}\right] \\
  & + \left[1-P_S(o(a) = 0|b_\hist, a)\right] \times \left[ \underbrace{R_E(b_\hist, a)}_{5.} + \min_{a' \in \mathcal{A}(b_{\hist a o})} \underbrace{Q(\{\mathcal{A}^p, p_a, \hist a o\}, a')}_{4.} \right],
  \end{split}
\end{equation}
where the highlighted terms are defined as follows:
\begin{enumerate}
\item $D(p_r, p_f)$: the cost of traveling from $p_r$, the position of the agent in $\mathcal{A}^p$, to the position of the frontier $p_f$ (as specified by $a_{f,z,z'}$). When this motion occurs entirely within known space, Dijkstra's algorithm can be used as a heuristic to calculate this cost. \footnote{However, if the previous action in $\hist$ takes the agent out of the known map (e.g., if robot is considering the next action after it just found the fire extinguisher), we estimate this value using the previously computed success or failure costs.}

\item $P_S(o(a) = 1|b_\hist, a)$: the probability of success. With probability $P_S$, the outcome of taking subgoal $a$ will be successful ($o=1$), and the robot will transition to the desired state $z'$ in the \gls{dfa}.

\item $R_S(b_\hist,a)$: the expected cost of success. Suppose the robot succeeds in transitioning via the subgoal specified by action $a_{f,z,z'}$ with a probability $P_S$. Then, with probability $P_S$, we accrue an expected cost of traveling from the frontier point $p_g$ to some point in the map enabling this transition.

\item $Q(\{\mathcal{A}^p, p_a, \hist a o\}, a')$: the future expected cost. After taking action $a$, we consider a different action, $a' \in \mathcal{A}(b_{\hist a o})$. This term is computed recursively until all actions in $\mathcal{A}(b_{\hist a o}))$ have been exhausted, or an actions succeeds. When that happens, $\mathcal{A}(b_{\hist a o})$ reflects the new actions set from the new state in the \gls{dfa} given $\hist a o$.

\item $R_E(b_\hist, a)$: the exploration cost. In the event that the agent does not make the desired transition in the \gls{dfa}, we say that it instead \emph{explores} the space beyond the subgoal of interest. With probability $1-P_S$, the agent then accumulates an \emph{exploration cost}, the expected cost of trying to navigate to the goal via $a$.

%\item $Q(\{\mathcal{A}^p, p_f, \hist a o\}, a')$: the future expected cost after a failed action. After taking action $a$, we consider a different action, $a' \in \mathcal{A}(b_{\hist a o})$. This term is computed recursively until all actions in $\mathcal{A}(b_{\hist a o}))$ have been exhausted, or an actions succeeds. When that happens, $\mathcal{A}(b_{\hist a o})$ reflects the new actions set from the new state in the \gls{dfa} given $\hist a o$.
\end{enumerate}

In theory, one could use Eq.\ref{eq:ltl-subgoal-planning-equation} to recursively solve for the optimal action by computing the cost for every possible policy. Then, by searching through the set of policies, it would be possible to determine the policy of lowest expected cost.
%This is the strategy used in \cite{Stein2018}, albeit for a much smaller search problem. 
The branching factor from having potentially many possible transitions, this approach is intractable for nontrivial environments and specifications.

%To compute the cost of a single policy, every time the robot imagines taking an action, it must consider the both that the action might succeed or fail. For each of these outcomes, it then must consider if the next action succeeds or fails. For one policy, if we assume $L$ transitions are needed to reach an accepting state, and there are $|A|$ actions in the action set at every state in the \gls{dfa}, every policy has $\left(\frac{|A|^{L+1}-1}{|A|-1}\right)$ instances where the robot had to make a decision. Each time the robot reaches a new state in the \gls{dfa}, it can trying all available subgoals in any order, so each state has combinatorial complexity. By this reasoning, we can loosely bound the complexity of finding the optimal policy through search as: $\mathcal{O}\left(|A|!^{\left(\frac{|A|^{L}-1}{|A|-1}\right)}\right)$, where $|A|$ is the size of the largest action set, and $L$ is the length of the longest trace through the \gls{dfa}.

%and considering a history of actions and outcomes $\hist$. The robot can choose any action $a_{g,q} \in \mathcal{A}_{\hist} = \{G \times \Delta(z)\}$, where $g$ is a location from $G$, and $q$ is a transition from $\Delta(z)$, to add to $\hist$. Here, $G = \{F,K\}$ is the set of all frontiers and transitions that can be made in the known map $m$ from position $p$, and $\Delta(z)$ is the set of possible transitions from state $z$ in the \gls{dfa}. Note that if $a_{g,q}$ has been added to $\hist$ already, it cannot be added again. Now, we will consider how we might identify the optimal action for our robot given its task specification.


%\subsection{Defining the Action Set}
%\label{sec:sub-action-set}

%As the robot moves through its environment, it must determine how to travel in order to satisfy its specification in minimum time. Because the task is accomplished when the robot reaches an accepting state, we are interested in taking ``high-level'' actions --- subgoals --- which attempt to advance the agent toward such a state in the \gls{dfa}.

%We consider three (3) different types of subgoals to define the set of actions available to the robot at a given time. This set depends on the state of the map, the state of the robot in the \gls{dfa}, and what subgoals the robot has already taken in its history. First, the robot can travel to a region of the known map which advances its state in the \gls{dfa} toward an accepting state. For example, if the robot has already revealed the fire extinguisher with its sensors, one subgoal would be to travel to the extinguisher's position in the map while avoiding any regions marked by fire (or any other regions in the map which would cause a different transition in the \gls{dfa}. This action would have a probability of success of one (1) if such a path exists, and the exact cost of success would be known by planning through the known map. For this case, we would not need to consider the possibility of the action failing.

%Second, the robot can attempt to advance its state in the \gls{dfa} by entering the unknown space beyond a particular frontier in an attempt to reach labeled region it has not yet revealed. For example, if the robot has not yet found the sprinklers, it could choose any of the frontiers that define the contiguous boundaries between free and unknown space, and travel through that frontier with the intent of finding the sprinklers while avoiding the fire (or making any other transitions). The probability of this subgoal successfully transitioning the \gls{dfa} state depends on the unknown portion of the map, and is estimated by the neural network. Similarly, the costs of success and failure are also estimated by the network. Note that the action of attempting to find the sprinklers beyond the same frontier is a different subgoal entirely, with different associated costs and probability of success.

%Finally, both because actions can fail to make the desired transition, and because multiple transitions may be necessary to reach an accepting state, the robot must consider histories of actions with multiple steps in order to succeed in its task. When considering future steps of a history, the robot also may consider taking actions beyond a frontier it has already chosen to explore earlier in a history. For example, if the robot is considering choosing a particular frontier in order to find the extinguisher without passing through the fire, it would then need to consider transitioning to the fire after it has found the extinguisher. Similarly, if the agent fails to find the extinguisher beyond a particular frontier, both the sprinklers and fire may still exist beyond that frontier. The set of available subgoals must reflect these actions for exploring beyond a frontier for alternate purposes. The probability of success for these actions is given by the neural network as before, though the costs of success and failure are calculated somewhat differently\footnote{explain here ...}. It is important to note that if the robot imagines an action failing in a history, it cannot take that action twice, and so removes it from its action set. This will be discussed in greater detail in section \ref{sub:mcts}.

%Consider a robot at position $p$, having revealed the partial map $m$, in state $z$ of the \gls{dfa}, and considering a history of actions and outcomes $\hist$. The robot can choose any action $a_{g,q} \in \mathcal{A}_{\hist} = \{G \times \Delta(z)\}$, where $g$ is a location from $G$, and $q$ is a transition from $\Delta(z)$, to add to $\hist$. Here, $G = \{F,K\}$ is the set of all frontiers and transitions that can be made in the known map $m$ from position $p$, and $\Delta(z)$ is the set of possible transitions from state $z$ in the \gls{dfa}. Note that if $a_{g,q}$ has been added to $\hist$ already, it cannot be added again. Now, we will consider how we might identify the optimal action for our robot given its task specification.


%\subsection{Computing the Cost of a Policy with Search}
%\label{sub:computing-cost}

%We define a policy $\Pi$ as a binary tree of subgoals, where each subgoal has some probability of successfully transitioning to its desired state in the \gls{dfa}, a cost associated with making that transition, and a cost of attempting to transition, and failing. Because each action is not deterministic, a policy must account for every contingency as the robot explores, so the branching factor of $\Pi$ is two (2). In other words, after selecting a subgoal, the robot must choose the next subgoal both for the case where that action succeeds --- the robot transitions to the desired state in the \gls{dfa} --- and when it fails. At each decision, we define the belief state $b_\hist = \{m, z, p_{r}, \hist\}$, which encapsulates the map state $m$, the \gls{dfa} state $z$, the robot position $p_{r}$, and the history of actions and outcomes $\hist$.

%Consider a robot at position $p$, having revealed the partial map $M$, and in state $z$ of the \gls{dfa}. At the root node of the policy, the robot picks an action $a_{g,q} \in \mathcal{A}(b^\tau_\hist)$, where $g \in M$ is a position selected from the set of frontiers and labeled regions in the known map, and $q \in \Delta(z^\tau_\hist)$ is a state in the \gls{dfa} the agent can transition to from the current state. $\hist$ is the ordered list of actions chosen to up to step $\tau$ in the current branch of $\Pi$ coupled with an indication of if they have been hallucinated to succeed or not (for $\tau = 0$, $\hist$ is empty). Because an action may succeed or fail, and because the set of actions available to the agent depends on past actions, the agent must keep track as it plans. If the robot hallucinates that its chosen action succeeds, the set $M$ does not change, but $z$ changes to reflect the new state in the \gls{dfa}. The robot cannot take the same action twice in a given $\hist$ however, so every time the robot imagines an action failing, its action set from that state is reduced by one, i.e. $\mathcal{A}(b_\hist^{\tau+1}) = \mathcal{A}(b_\hist^{\tau}) \setminus a_{g,p}$. Stated differently, any particular $a_{g,q}$ can only be chosen once per $\hist$.

\begin{comment}


\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/need_memory_in_algorithm.png}
\caption{$\lozenge((a \wedge \lnot b) \wedge \lozenge((b \wedge \lnot a) \wedge \lozenge(a \wedge \lnot b)))$}\label{fig:need_memory_in_algorithm}
\end{figure}


\hkc{this is really notation heavy and I am not sure all of this is needed. I also do not understand why there is a "plan" and a "DFA". seems to me they represent the same thing. a few random other things: why do we need p (position)? why do we have $z_\hist$? why is $\delta$ defined here again? }
Notation for action/\gls{dfa} transition pairs:
\begin{flushitemize}
\item $Q(b^\tau_\hist, a_{g,q})$ = cost of taking action $a_{g,q}$ in belief state $b^\tau_\hist$
\item $b^\tau_\hist = \{M, \hist\}$ = current belief state
\item $M$ = the current map
\item $\hist = (a_1, sf_1) (a_2, sf_2) (a_3, sf_3) ... (a_\tau, sf_\tau)$ = history of actions and success/failure record ($sf_i \in \mathbb{B}$) chosen up to step $\tau$
\item $a_{g,q} \in \mathcal{A}(b_\hist^\tau)$ = action to explore a frontier to find the proposition that will transition to state $q$ in the \gls{dfa}
\item $p$ = position of robot
\item $g \in M$ = a frontier/subgoal
\item $z^{\tau+1}_\hist$ = state in \gls{dfa} the robot is in at step $\tau+1$
\item $\delta: Z x \Sigma \rightarrow Z$ = transition function in \gls{dfa}
\item $\Delta(z) = \{z' \ |\ \exists \sigma \in \Sigma\ \textrm{s.t.}\ z' = \delta(z,\sigma)\}$ potential next states in the \gls{dfa} from state $z$
\item $q \in \Delta(z^\tau_\hist)$ = potential state in the \gls{dfa} that the robot wants to transition to
\item $P_S(z^{\tau+1}_{\hist}=q|b_\hist^\tau,a_{g,q})$ = probability of reaching state $q$ in the \gls{dfa} given a frontier $a_g$
\item $R_S(b_\hist^\tau,a_{g,q})$ = success cost of reaching state $q$ in the \gls{dfa} given a frontier $a_g$
\item $R_E(b_\hist^\tau,a_{g,q})$ = exploration cost of not reaching state $q$ in the \gls{dfa} given a frontier $a_g$
\end{flushitemize}
\end{comment}


%The cost of choosing subgoal $a_{g,p}$ from belief $b_\hist$, then following the optimal policy $\Pi$ is defined below:

% \begin{equation}\label{eq:ltl-subgoal-planning-equation}
%  \begin{split}
%  Q&(b_\hist, a_{g,q}) = \underbrace{D(m, p_r, p_g)}_{1.} + \\
%  & \underbrace{P_S(z_{\hist a_{g,q}} = q|b_\hist, a_{g,q})}_{2.} \times \\
%  & \left[\underbrace{R_S(b_\hist,a_{g,q})}_{3.} + \min_{a \in \mathcal{A}(b_{\hist a_{g,q}})} %\underbrace{Q(\{m, q, g, \hist\}, a)}_{5.}\right] + \\
%  & \left[1-P_S(z_{\hist a_{g,q}} = q|b_\hist, a_{g,q}))\right] \times \\
%  & \left[ \underbrace{R_E(b_\hist, a_{g,q})}_{4.} + \min_{a \in \mathcal{A}(b_{\hist a_{g,q}})} %\underbrace{Q(\{m, z, g, \hist\}, a)}_{5.} \right],
%  \end{split}
%\end{equation}



%There are two important observations we can note which must be, and are in fact true about this cost. First, in the case where the task specification is simple, goal-directed search, the cost calculation reduces to the same as in \cite{Stein2018}. This supports our claim that we are presented a more general form of learned subgoal planning. Second, we note that in the case where the map is fully observable, equation \ref{eq:ltl-subgoal-planning-equation} is optimal (minimizes travel cost) for the given specification.



\subsection{Computing cost using PO-UCT}
\label{sub:mcts}
Exhaustive search is impractical for a problem of this complexity. Fortunately however, it is not necessary. We have structured our learning problem such that, given a subgoal as an input, our network estimates the probability that the action succeeds, as well as the cost of that action for either outcome. This is discussed further in Sec. \ref{sec:learning}. With this model, we use \gls{pouct}, a generalization of \gls{mcts} which keeps track of histories of actions and outcomes, to select the optimal action \citet{POMCP}. The nodes of our search tree correspond to belief states $b_\hist$, and actions available at each node are defined in Sec.~\ref{sec:sub-action-set}. \gls{pouct} is well suited to our problem setting, prioritizing the most promising branches of the search space and greatly reducing the complexity of the cost calculation during planning.

%The nodes of our search tree correspond to belief states $b_\hist$, and each node contains a value $V(b_\hist,a)$, and a visitation count $N(b_\hist,a)$. The procedure for growing and refining a \gls{pouct} tree is to begin at the root node ($b_{\hist_0}$), and pick the most promising action according to:
%\begin{equation}\label{eq:po-uct}
%V(b_\hist,a)^* = V(b_\hist,a) + c\sqrt{\frac{log(N(b_\hist))}{N(b_\hist,a)}},
%\end{equation}
%where $N(b_\hist)$ corresponds to the number of time we have seen that node in simulations, and $N(b_\hist,a)$ is how often we have seen that node and chosen action $a$. The second term in the above equation captures the relative ratio of exploration and exploitation, and is modulated by the scalar $c$. One impact of this term is that all actions from a particular node are simulated at least once before any are tried a second time.

% \gls{pouct} is particularly well suited to our problem for three reasons. First, it enables the agent to greatly reduce the complexity of the cost calculation by ignoring low probability regions in the policy tree which do not contribute in a meaningful way to cost of the policy. The most promising branches are explored most often, leading their inputs to be more accurately valued.  Second it requires a generative model of the outcomes and costs of different actions, which we get from trained network. Finally, the set of possible outcomes from our subgoals is discrete and small (either a subgoal succeeds or it doesn't). Therefore, we don't suffer from the infinitely large branching factors partially observable problems usually face in continuous domains. 

%\gls{mcts} is a probabilistic sampling technique which allows the agent to to greatly reduce the complexity of the cost calculation by ignoring low probability regions in the policy tree which do not contribute in a meaningful way to cost of the policy. Traditionally, \gls{mcts} relies on a state-based representation which does not need to keep track of the history of actions in a plan. Since the subgoals available to our agent depend on previous actions in a proposed sequence however, \gls{pouct} as presented by Silver and Veness \cite{POMCP} is better suited for our application. 



%Best first search according \eqref{eq:po-uct} will continue through the tree until a node has been selected which has not yet been simulated. From there, a sequence of actions is randomly selected according to some policy (often uniformly random) until either the agent simulates reaching an accepting state, or no actions are available and the robot fails (accruing some additional cost). This is called the rollout step, after which, all costs are propagated back up the tree to update the $V(b,a)$ and $N(b,a)$ values of parent nodes until the root is reached. \gls{pouct} is an anytime algorithm, so once a pre-defined amount of time has passed, we stop simulating, and the action with the highest $Q(b,a)$ from the root node is chosen. Additionally, like \gls{mcts}, \gls{pouct} is asymptotically optimal, meaning if we simulate for long enough, we should expect to return the optimal action according to \eqref{eq:ltl-subgoal-planning-equation}.



% \subsection{Computing Costs in Known Space}
% \adam{Note that this section needs references and notation}
% We can take advantage of existing methods for planning with \gls{scltl} specifications in known maps to alleviate the computational complexity of our approach. Given the explored map and the \gls{dfa} representing the \gls{scltl} specification, we can create a product automaton \cite{}. If the specification were realizable, we could search the product automaton to find the shorted path to an accepting state. 

% However, when the specification is not realizable, we can leverage the product automaton to find the shortest path to frontier states that make progress in the \gls{dfa}. Since we are interested in finding the minimum cost path, we want to find the shortest cost path to the frontier. However, we also want to progress in the \gls{dfa}. We therefore find the minimum cost path to reach each \gls{dfa} state (if possible) at each frontier. 

% Once the planning algorithm has hallucinated exploring a frontier and returning to known space with an updated \gls{dfa} state, we can once again use the known product automaton to find the shortest path to every possible \gls{dfa} state at every frontier.

\section{Learning Transition Probabilities and Rewards}
\label{sec:learning}

\gls{pouct} requires a generative model in order to compute cost, implying our network must be able to estimate three properties (as defined in \eqref{eq:ltl-subgoal-planning-equation}) of each possible subgoal $a_{f,z,z'}$. For each frontier $f$, we want to estimate $P_S$, $R_S$, and $R_E$ for the transition between a chosen $z$ and $z'$. In this section, we discuss how we structure our learning objective and estimate the properties we need for planning.
% Even in our firefighting example, we need to to estimate probabilities and costs for many different combinations of transitions and frontiers.\todo{should/can we put a number with this with the figure of a partially explored environment?}

\subsection{Encoding a Transition}
\label{sub:encoding}
As discussed previously, our model requires a finite-sized vector to encode which transition we care about as input to our neural network. We assume the robot knows which propositions are relevant for completing any of the tasks we might assign it as defined by $\Sigma$. For the burning building example, $\Sigma = \{\texttt{fire}, \texttt{outside}, \texttt{alarm}, \texttt{extinguisher} \}$. Depending on the \gls{dfa} and the robot's state in it, a transition can occur if the robot enters a state in the \gls{wfdts} where the propositions have a particular assignment of either true or false according the the labeling function $l: S \rightarrow 2^\Sigma$. For a given transition to occur, certain propositions must be true, certain propositions must be false, and certain propositions can be either. If the robot plans a path through the product automaton $\mathcal{A}^P$ which transitions to a new state in the \gls{dfa}, then until that transition, the agent must remain in it's original state via self-transitions. For this to happen it can only enter states in the \gls{wfdts} whose labels cause a self-transition and not a transition into some other new state in the \gls{dfa}. Therefore, propositions have a specific true, false, or either assignment for path to a transition as well.

For a problem in which there are $n$ atomic proposition of interest, we can thus define 2 $n$-dimensional vectors (one for the path to a transition, and one for the transition itself) where each element corresponds to a proposition. A proposition either must be false (-1: do \emph{not} pass through the fire), must be true (1: the robot must be in a grid cell that contains an extinguisher), or can be either (0: it does not matter if the robot goes to the exit at this time). We use these vectors as input to our neural network to encode what the agent must do to stay in its current \gls{dfa} state, and to indicate which transition we are interested in making for a particular subgoal. Further description of this network is given below. 
%There are a few ways this could be accomplished, but perhaps the simplest (and the one implemented in this work), is presented below. 


%For each transition, we can imagine a trajectory composed of two components: the portion where the robot has not yet transitioned from its current state in the \gls{dfa}, and the last step in the trajectory, where it makes the transition to the desired state. In the pre-transition component of the trajectory, the robot must not leave the state it is in, and the final step must take it to its new state. Our goal is to find a way to represent these two components of a transition as a vector to input to a neural network.

%For a problem in which there are $n$ atomic proposition of interest, we define 2 $n$-dimensional vectors, one for each component of a trajectory, where each element corresponds to a proposition. For our running example, we will have element 0 represent extinguisher, element 1 represent sprinkler, element 2 represent exit, and element 3 represent fire. In both the components of a trajectory, there are three ways we could consider a proposition for a given transition, which correspond to a value of either -1, 1, or 0 in a vector. A proposition either must be false (-1: do \emph{not} pass through the fire), must be true (1: the robot must be in a grid cell that contains an extinguisher), or can be either (0: it does not matter if the robot goes to the exit). These values will not be the same for both components of a trajectory. 
%For example, if the transition of interest is to find the extinguisher without passing through the fire, the first 

%As an example, if our fire-fighting robot is considering a transition that finds the extinguisher while avoiding the fire, the first component of this transition vector would be: $[-1, -1, 0, -1]$ and the second: $[1, -1, 0, -1]$. Then, if the robot wants to transition to the fire, the two vectors would be: $[0, -1, 0, -1]$, and $[0, 0, 0, 1]$. We get the first vector from the self-transitions for the current state in the \gls{dfa}, and get the second vector from the transition of interest. By virtue of being of a constant dimension, we can use these vectors as input to our neural network (defined below) to encode the transition for a given subgoal.

%As the robot attempts to make a transition in the DFA, it must not leave it's current state until it can make the transition in one step. As such, when the robot is traveling, a proposition either must be false (do \emph{not} pass through the fire), must be true (the robot must stay in the hallway), or can be either (it doesn't matter if the robot goes to the exit along the way). Then, at the end of a trajectory, the robot must make it's transition. As with the trajectory, there are regions it must enter (it must enter a grid cell that has an extinguisher), regions it cannot enter (once again, do not enter a grid cell that has fire), and regions that are irrelevant.

%There are three ways we could consider a proposition in a given transition. We may want the proposition to be true (go to the extinguisher), we may want the proposition to be false (do \emph{not} pass through the fire), or it may not be relevant for this transition (it doesn't matter if the robot goes to the exit along the way).
%There are three ways we could consider a proposition in a given transition. We may want the proposition to be true (go to the extinguisher), we may want the proposition to be false (do \emph{not} pass through the fire), or it may not be relevant for this transition (it doesn't matter if the robot goes to the exit along the way). As such, we define a positive one in the vector to mean the proposition must be true, a negative one to mean false, and zero to mean it is not relevant.

\subsection{Network Architecture}
\label{sub:architecture}
As it was for the original Learned Subgoal Planning work, the output of our network is of three channels; one for each property of the subgoal. The input to the network is an RGB image taken from a panoramic camera and the transition vectors as defined above.

%The input to the network is an RGB image taken from a panoramic camera, the relative position of the chosen subgoal to the camera, and the transition vectors as defined above.

The network takes a $128\!\times\!512$ pixel RGB panoramic image and $2 1\!\times\!n$ vectors describing the transition of interest, and returns the three properties over a $32\!\times\!128$ grid, where each point corresponds to a range-bearing coordinate from the sensor. We use a fully-convolutional encoder-decoder network structure composed of blocks. Each encoder block consists of two convolution layers with $3\!\times\!3$ kernels, followed by a batch norm operation and a ReLU activation function, and terminated by a $2\!\times\!2$ max-pooling operation. Decoder blocks are similar, however the final convolutional layer has stride 2 (so that the output is upsampled) and the max-pooling operation is eliminated. The network consists of 5 encoder blocks, with output channels $[64, 64, 128, 128, 256]$, and 3 decoder blocks, with output channels $[128, 64, 64]$. The image is the only input at the first layer of the encoder. After the first encoder block, we concatenate the transition vectors to each element, and continue encoding. The output of the final decoder layer is passed through a final $1\!\times\!1$ convolutional layer with three output channels, corresponding to the three properties of the subgoals. We use a cross entropy loss to train our network, which is weighted as in \citet{Stein2018} with a heuristic computed to account for the cost of mis-classifying a subgoal. The Adam optimizer is used to train the network for 200k steps, with an initial learning rate of 0.005 and a learning rate decay of 0.5 every 10k steps.

%A weighted cross-entropy with an empirically chosen positive-weight is used  as the loss function for the vertex likelihood, so that the sparse positive detections are not overwhelmed by the  negative  background.

\subsection{Generating Training Data}
We train our network using data generated in simulation. Using the Unity game engine, we build multiple different environments from the same distribution in which our simulated robot can navigate from point to point. After the robot travels a short distance, a panoramic image is taken, all possible subgoals given the propositions in the environment are identified, and the three properties ($P_S$, $R_S$, and $R_E$) are computed from the ground truth map for each of the possible transitions. For each new environment class we consider (e.g. school vs apartment), we train a new network. However, we can use the same network within the same environment class for different tasks.


%ADAM
\subsection{High-Level Actions}


Since, the map is only partially known, the agent needs to know how to behave in known space and anticipate the consequences of its actions in unknown space.
Inspired by \citet{Stein2018}, we define \textit{frontiers} as the contiguous boundaries between known space and unknown space.
We split the behavior of the robot into what happens before it reaches the frontier and what happens after it passes through the frontier into unknown space.
% As the \gls{dfa} can be used to track the progress of the agent and determine what future
We define the \gls{dfa} state $z$ as the state of the robot when it reaches the frontier and $z'$ as the state the robot plans to be in after exploring beyond the frontier $f$.
A \textit{high-level action} is then defined as:

\begin{equation}
    a_{f,z,z'} = (f, z, z')
\end{equation}

For example, in Fig. \ref{fig:defining-actions}, the agent could travel through frontier $f_1$ by going straight to it, or traveling through region A first, resulting in high-level actions $a_{f_1,1,0}$ and $a_{f_1,2,1}$.

For a given set of frontiers $\mathcal{F}$ and \gls{dfa} state, we define the set of all high-level actions as:

\begin{equation}
    \mathcal{A}(z_{current},\mathcal{F}) = \{a_{f,z,z'} | f \in \mathcal{F}, z \in Reachable(z_{current} \setminus F, \exists \sigma \textrm{s.t.} z' = \delta_{A}(z, \sigma) \}
\end{equation}

where $Reachable(z_{current}) = \{All dfa states that are reachable from z_{current}\}$.

Note that the set of high-level actions also includes actions where for $a_{f,z,z'}$, $z$ can't be achieved by traveling in known space, but is only possible by making a transition in the \gls{dfa} in unknown space.

As in \cite{Stein2018}, we check if the task can be completed in known space and add that to our set of high-level actions. \adam{Why are we switching to use subgoals vs sticking with high-level actions again?}

% \begin{flushitemize}
% \item Action $a$ has outcome $o$, history of these actions $h$
% \item $b_h$ contains the robot's belief - where it is and what it can observe $\{p_a, hoa, sensors\}$ - the product automaton state fully encompases where the robot is in the world and the dfa state
% % \item Belief history $b_h$ encompasses what the robot observes about the world $b_h = \{A^P, p_a, hoa\}$
% \item Likelihood of success
% \item Associated cost of success or failure in unknown space
% \item Remove/Modify action list
% \item Cost of traveling to the frontier
% \item Expected cost of an action - whole formula
% \end{flushitemize}

% As our objective is to find the minimum cost path to satisfy a specification, we need to consider the likelihood of success and expected cost of each high-level action, along with the order to attempt them.

% We denote the outcome of an action $a_{f,z,z'}$ as $o(a_{f,z,z'}) \in \{0,1\}$ where $0$ indicates the action failed and $1$ that it succeeded.
% This history is encompassed in $h = \{a_0, o(a_0), $


% Consider a robot at state $p = (s,z)$ in the product automaton $s$ in the \gls{lts} and state $z$ in the \gls{dfa}, planning to reach an accepting state in the \gls{dfa}.

